Rigid equivalences of $5$-dimensional $2$-nondegenerate rigid real hypersurfaces $M^5 \subset \mathbb{C}^ 3$ of constant Levi rank $1$

We study the local equivalence problem for real-analytic ($\mathcal{C}^\omega$) hypersurfaces $M^5 \subset \mathbb{C}^3$ which, in coordinates $(z_1, z_2, w) \in \mathbb{C}^3$ with $w = u+i\, v$, are rigid: \[ u \,=\, F\big(z_1,z_2,\overline{z}_1,\overline{z}_2\big), \] with $F$ independent of $v$. Specifically, we study the group ${\sf Hol}_{\sf rigid}(M)$ of rigid local biholomorphic transformations of the form: \[ \big(z_1,z_2,w\big) \longmapsto \Big( f_1(z_1,z_2), f_2(z_1,z_2), a\,w + g(z_1,z_2) \Big), \] where $a \in \mathbb{R} \backslash \{0\}$ and $\frac{D(f_1,f_2)}{D(z_1,z_2)} \neq 0$, which preserve rigidity of hypersurfaces. After performing a Cartan-type reduction to an appropriate $\{e\}$-structure, we find exactly two primary invariants $I_0$ and $V_0$, which we express explicitly in terms of the $5$-jet of the graphing function $F$ of $M$. The identical vanishing $0 \equiv I_0 \big( J^5F \big) \equiv V_0 \big( J^5F \big)$ then provides a necessary and sufficient condition for $M$ to be locally rigidly-biholomorphic to the known model hypersurface: \[ M_{\sf LC} \colon \ \ \ \ \ u \,=\, \frac{z_1\,\overline{z}_1 +\frac{1}{2}\,z_1^2\overline{z}_2 +\frac{1}{2}\,\overline{z}_1^2z_2}{ 1-z_2\overline{z}_2}. \] We establish that $\dim\, {\sf Hol}_{\sf rigid} (M) \leq 7 = \dim\, {\sf Hol}_{\sf rigid} \big( M_{\sf LC} \big)$ always. If one of these two primary invariants $I_0 \not\equiv 0$ or $V_0 \not\equiv 0$ does not vanish identically, we show that this rigid equivalence problem between rigid hypersurfaces reduces to an equivalence problem for a certain $5$-dimensional $\{e\}$-structure on $M$.

==> title-author <==
$\:$

\bigskip\bigskip\bigskip\bigskip\bigskip

\begin{center}

{\large\bf
Rigid equivalence problem for 5-dimensional 2-nondegenerate \\ rigid real hypersurfaces $M^{5}\subseteq \mathbb{C}^{3}$ of constant Levi-rank 1}
\label{immersion-bidisk}

\bigskip\bigskip

Wei Guo {\sc Foo},\qquad Jo\"{e}l {\sc Merker}\footnote{This work was supported in part by the Polish National Science Centre (NCN) via the grant number 2019/29/B/ST1/02583}, \qquad The-Anh {\sc Ta}

\smallskip

%{\large\footnotesize\sf D\'epartement de Math\'ematiques d'Orsay}

%{\large\footnotesize\sf Université Paris-Sud, France}

\end{center}\bigskip

\bigskip


==> write.tex <==

%%% PARIS %%%

\setlength{\textheight}{12.05cm}
\setlength{\textwidth}{14.05cm}
\voffset -4.05cm
\hoffset -4.25cm

%%% AVANNE %%%

%\setlength{\textheight}{13.5cm}
%\voffset -3.85cm
%\hoffset -4.25cm


